DeepView: View Synthesis with Learned Gradient Descent

We present a novel approach to view synthesis using multiplane images (MPIs). Building on recent advances in learned gradient descent, our algorithm generates an MPI from a set of sparse camera viewpoints. The resulting method incorporates occlusion reasoning, improving performance on challenging scene features such as object boundaries, lighting reflections, thin structures, and scenes with high depth complexity. We show that our method achieves high-quality, state-of-the-art results on two datasets: the Kalantari light field dataset, and a new camera array dataset, Spaces, which we make publicly available.

==> datasets.tex <==



==> old-intro.tex <==
\section{Introduction}

Light fields offer a compelling way to view scenes from a continuous, dynamic set of viewpoints. However, creating light fields for real scenes from a sparse set of captured images is a long-standing challenge. Part of this challenge is that the problem is inherently ill-posed: a light field is a 4D function that we wish to reconstruct from sparse 2D views. Accordingly, light field reconstruction is an \textit{inverse problem}, like computed tomography (CT) or image deblurring, where we want to reconstruct a model with a number of parameters that is much larger than the effective number of measurements. Such inverse problems can be solved via optimization methods like gradient descent, that solve for the parameters that best predict the measurements via a forward model like a renderer. However, for ill-posed problems such optimizers very easily overfit the measurements, necessitating the use of priors that are difficult to design by hand. In the case of view synthesis, such overfitting is evident in interpolated views with noticeable artifacts.

We present a new method for solving for light fields from sparse views that uses \emph{learned gradient descent} and achieves state-of-the-art view synthesis results without noticeable artifacts. 
Building on recent ideas from the optimization community~\cite{XYZ}, our learned gradient descent replaces the simple gradient descent update rule with a deep network that processes the gradients to generate the parameter update.  The use of a network in the update rule allows for a learned prior on the model parameters, enforced by manipulating the gradients. Additionally, the network can learn to take larger,  parameter specific steps than standard gradient descent. The use of the gradients as input to the network instead of the original measurements efficiently delivers the information from the measurements to the model parameters that affect them, removing the need for dense network connections.


The classic approach to such inverse problems is to solve an optimization problem that considers the model’s ability to predict the measurements using a forward operator like a renderer. When the problem is under-constrained there are many models that explain the measurements well and a prior is used to select the ``best'' of these models. Optimization based methods are efficient in the sense that, through the gradient, they directly couple the measurements and the typically small set of model parameters that affect them. In practice, devising good priors and solving the optimization problem efficiently are very challenging.

The rise of deep learning presents an alternative: train a deep network to directly predict a model from input measurements. Relatively simple feed-forward networks can generalize well, particularly for problems where there is a simple relationship between the input measurements and output model parameters. For example, in image deblurring, to estimate a pixel in the original image we only need access to a small neighborhood of pixels in the blurred image, convolutional network are designed to process such neighborhoods. 
However, for many problems there is no such simple relationship between the measurements and model parameters. This is especially true for stereo and view synthesis where the depth or color of a scene point depends on both the geometric relationship between the input views as well as interactions within the solved scene itself, since one part of a scene can occluded another part of the scene in some of the views. One way to solve these types of problems is through the use of fully connected networks, where e.g.\ every input pixel is connected to every pixel of the novel view. However, the large number of parameters in such a network makes it impractical even at low resolutions.
To partially solve this problem for view synthesis we can present the input images to the network as plane sweep volumes, which implicitly model the geometric relationship between the different input and target views. This still leaves the visibility problem, which is naively handled by adding connections across depth planes. These across-depth connections quickly become unwieldly, for example a 3D convolution kernel with a 3x3 pixel neighborhood and 64 depth planes has many parameters and is both expensive and prone to overfitting.

Recently the optimization community has developed methods that combine the best of both the optimization and learning based approaches using techniques known as \emph{learned gradient descent}~\cite{}. Learned gradient descent replaces the simple gradient descent update rule with a deep network that processes the gradients to generate the parameter update.  The use of a network in the update rule allows for a learned prior on the model parameters, enforced by manipulating the gradients. Additionally, the network can learn to take larger,  parameter specific steps than standard gradient descent. The use of the gradients as input to the network instead of the original measurements efficiently delivers the information from the measurements to the model parameters that affect them, removing the need for dense network connections. 

In this work we present a method for predicting light fields from data that leverages these learned gradient descent methods. For our scene representation we build on the recent idea of representing light fields as stacks of colored, semi-transparent planar layers~\cite{wetzstein,zhou}, which can represent complex scenes effectively, but are highly overparameterized. We adapt the learned gradient descent technique to infer the parameters of these layers. We show that for this problem the gradients have a particular intuitive form in that they encode the visibility information between the views and the layers. By explicitly modelling visibility our method shows improved performance in traditionally difficult areas such as edges and regions of high depth complexity.
In addition to the method itself, we also present a large, challenging new dataset of light field captures suitable for training and testing view synthesis models.


\author{John Flynn}
\affiliation{\institution{Google Inc.}}
\email{jflynn@google.com}

\author{Michael Broxton}
\affiliation{\institution{Google Inc.}}
\email{broxton@google.com}

\author{Paul Debevec}
\affiliation{\institution{Google Inc.}}
\email{debevec@google.com}

\author{Matthew Duval}
\affiliation{\institution{Google Inc.}}
\email{matthewduval@google.com}

\author{Graham Fyffe}
\affiliation{\institution{Google Inc.}}
\email{fyffe@google.com}

\author{Ryan Overbeck}
\affiliation{\institution{Google Inc.}}
\email{rover@google.com}

\author{Noah Snavely}
\affiliation{\institution{Google Inc.}}
\email{snavely@google.com}

\author{Richard Tucker}
\affiliation{ \institution{Google Inc.}}
\email{richardt@google.com}
